Strangeness-changing scalar form factors

We derive expressions for strangeness-changing scalar form factors, which incorporate known theoretical constraints both at low and high energies. Their leading behaviour in the limit of a large number of colours is calculated from the resonance chiral Lagrangian. A set of short-distance constraints on the scalar resonance couplings is obtained, imposing the form factors to vanish at infinite momentum transfer. Making use of previous results on S-wave KPi scattering [1], and a coupled--channel dispersion-relation analysis, the KPi, KEta and KEta' scalar form factors are calculated up to 2 GeV. These scalar form factors are a key ingredient in the determination of the corresponding scalar spectral function which is important in the extraction of the mass of the strange quark from QCD sum rules as well as hadronic tau decays.

==> mathematica.tex <==
% File mathematica.tex -- TeX/LaTeX mma common code
% Macros for TeX/Mathematica documents
% Written 2/26/1991 by Dan Dill dan@chem.bu.edu


% Copyright (C) 1991 Dan Dill
% This is part of TeX/Mathematica
%
% TeX/Mathematica is distributed in the hope that it will be useful, but
% WITHOUT ANY WARRANTY.  No author or distributor accepts responsibility to
% anyone for the consequences of using it or for whether it serves any
% particular purpose or works at all, unless he says so in writing.
%
% Everyone is granted permission to copy, modify and redistribute this
% file, provided:
%  1.  All copies contain this copyright notice.
%  2.  All modified copies shall carry a prominant notice stating who
%      made the last modification and the date of such modification.
%  3.  No charge is made for this software or works derived from it.  
%      This clause shall not be construed as constraining other software
%      distributed on the same medium as this software, nor is a
%      distribution fee considered a charge.
%
% The right to distribute this file for profit or as part of any commercial
% product is specifically reserved for the author.



\everyjob{\typeout{TeX/Mathematica `mathematica.tex' Version 1.2 <Mon Feb 25 1991>}}
\immediate\write10{TeX/Mathematica `mathematica.tex' Version 1.2 <Mon Feb 25 1991>}

% Left indentation
\def\mmaindent#1{\gdef\@mmaindent{#1}}
%\gdef\@mmaindent{\z@}
\gdef\@mmaindent{\parindent}


% Verbatim setup
% This handles leading spaces on a line, spaces after ., etc. TeXbook p. 352, 421
{\obeyspaces\gdef {\ }} % \obeyspaces now give \ , not \space
\def\uncatcodespecials{\def\do##1{\catcode`##1=12 }\dospecials}
\def\setupverbatim{%
	\v@rbsize
	\def\par{\leavevmode\egroup\box0\endgraf}
	\obeylines \uncatcodespecials
	\obeyspaces
	\catcode`\`=\active \catcode`\^^I=\active
	\catcode`\`=12
	\everypar{\startbox}}


% Tab expansion
\def\startbox{\setbox0=\hbox\bgroup}  % The box is width \the\w.
{\catcode`\^^I=\active % Don't use <tab> for the rest of this text!
 \gdef^^I{\leavevmode\egroup
   \dimen0=\wd0 % width so far, or since previous tab
   \divide\dimen0 by\w
   \multiply\dimen0 by\w % compute previous multiple of \w
   \advance\dimen0 by\w % advance to next multiple of \w
   \wd0=\dimen0 \box0 \startbox}}


% This hack discards CR after \begin{mma}... to prevent a blank line at the start
% of cells.  It works (I think) because TeX reads past the CR in getting the
% "next token" for \futurelet.
\def\@mma{\futurelet\nextchar\@@@mma}

\def\@@@mma{\mm@setdims
	\let\mm@tail = \mm@end % May have more than one end in future
	\ifx\nextchar [%
		\let\next = \@mmainit
	\else
		\let\mm@head = \mm@start
		\let\next = \@@mma
	\fi \next}

\def\@mmainit[#1]{% Just gobble up argument for now.  Examine when more options
	\let\mm@head = \mm@startinit
	\futurelet\nextchar% Gobble up CR if any
	\@@mma}




\def\@@mma{\bigbreak
	\mm@head
	\begingroup
		\parindent=\@mmaindent % Indent listing
		\setupverbatim
		\doverbatim}


% \end{mathematica}
\begingroup
% Redefine grouping characters, so {...} can delimit macro
\catcode `\{=12 \catcode `\}=12 \catcode `[=1 \catcode `]=2
% Redefine escape, so \end can be a macro delimiter
\catcode`\|=0 \catcode`\\=12 % | is temporary escape character
	|obeylines|gdef|doverbatim#1\end{mathematica}^^M%
					    %Gobble CR at end of \end{mathematica}
	[#1|endgroup|mm@tail|bigbreak|noindent]%
|endgroup

% Cell graphics
\def\mm@box#1{\hbox{\vrule\vbox{\hrule
	\hbox spread 1pt{\hfil\vbox to \mm@length{\vfil
		\hbox{\b@xfont #1}%
	\vfil}\hfil}
\hrule}\vrule}}
\def\mmabox#1{\mm@setdims\mm@box#1} % External version

% Dimensions for construction of cell headers/footer
\newdimen\texd@fht \texd@fht=.4pt % plain TeX default rule height
\newdimen\mm@length % Length of vertical tics on cell header/footer
\newdimen\mm@lengthhalf % One-half of vertical tic length
\newdimen\mm@lengthplus % Vertical tic length plus horizonatal rule height

% Execute for each cell in case font size has changed
\def\mm@setdims{
%\mm@length=\ht\strutbox \advance\mm@length by\dp\strutbox \divide\mm@length by 2
\mm@length=\baselineskip \divide\mm@length by 2
\mm@lengthhalf=\mm@length \divide\mm@lengthhalf by 2
\mm@lengthplus=\mm@length \advance\mm@lengthplus by \texd@fht
}

\def\mm@startinit{%
	\vskip -\mm@lengthhalf
	\hbox to \hsize{%
		\vrule height\texd@fht depth\mm@length
		\hrulefill
		\lower\mm@lengthplus\mm@box{I}}
	\vskip \mm@lengthhalf}
\def\mm@start{%
	\vskip -\mm@lengthhalf
	\hbox to \hsize{%
		\vrule height\texd@fht depth\mm@length
		\hrulefill
		\vrule height\texd@fht depth\mm@length}
	\vskip \mm@lengthhalf}
\def\mm@end{%
	\hbox to \hsize{%
		\vrule height\mm@lengthplus depth0pt
		\hrulefill
		\vrule height\mm@lengthplus depth0pt}}


% Setup psfig prolog --- for LaTeX/Mathematica graphics
% Assumes psfig.sty or psfig.tex
% This macro should be invoke after \begin{document} or \input psfig
% Edit the locations /usr8/dan/tex/inputs/ to those for your site
\def\psfiginit{%
% ArborText dvips
%\special{ps: plotfile /usr8/dan/tex/inputs/psfig.pro global}
%\special{ps: plotfile /usr8/dan/tex/inputs/mma.pro.1.2 global}
% Rokicki dvips
\special{header=/usr8/dan/tex/inputs/psfig.pro}
\special{header=/usr8/dan/tex/inputs/mma.pro.1.2}
}

